CAMEL-Bench: A Comprehensive Arabic LMM Benchmark

Recent years have witnessed a significant interest in developing large multimodal models (LMMs) capable of performing various visual reasoning and understanding tasks. This has led to the introduction of multiple LMM benchmarks to evaluate LMMs on different tasks. However, most existing LMM evaluation benchmarks are predominantly English-centric. In this work, we develop a comprehensive LMM evaluation benchmark for the Arabic language to represent a large population of over 400 million speakers. The proposed benchmark, named CAMEL-Bench, comprises eight diverse domains and 38 sub-domains including, multi-image understanding, complex visual perception, handwritten document understanding, video understanding, medical imaging, plant diseases, and remote sensing-based land use understanding to evaluate broad scenario generalizability. Our CAMEL-Bench comprises around 29,036 questions that are filtered from a larger pool of samples, where the quality is manually verified by native speakers to ensure reliable model assessment. We conduct evaluations of both closed-source, including GPT-4 series, and open-source LMMs. Our analysis reveals the need for substantial improvement, especially among the best open-source models, with even the closed-source GPT-4o achieving an overall score of 62%. Our benchmark and evaluation scripts are open-sourced.

==> Tables/CAMEL-Bench_facts.tex <==
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{5pt}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lllcccccc}
    \toprule
    Domain & Sub-domain & Existing Dataset & Web/Generated & Split & Original Language & Number of QA\\
    \midrule
    Multimodal Understanding & Visual understanding/Reasoning & MME & Dataset & Test & En & 1,389 \\
    \& Reasoning (15,934 QA) & & MMBench & Dataset & Dev & En & 2,291 \\
    & & MMT-MI-Bench & Dataset & Val & En & 662 \\
    & & SEED & Dataset & Test & En & 592 \\
    & & MMMU (Validation) & Dataset & Val & En & 718 \\
    & Object hallucination evaluation & CountBench & Dataset & Val & En & 344 \\
    & & MMT-MI-Bench & Dataset & Val & En & 186 \\
    & & POPE & Dataset & Test & En & 467 \\
    & Math and logic reasoning & MathVista & Dataset & Testmini & En & 531 \\
    & Scientific reasoning & ScienceQA-IMG & Dataset & Val & En & 801 \\
    & & Exams-V & Dataset & Test & AR & 823 \\
    & Visual Question Answering & GQA & Dataset & Val & En & 1,938 \\
    & & VizWiz & Dataset & Val & En & 999 \\
    & & VQAv2 & Dataset & Val & En & 903 \\
    & Infographics VQA & AI-Generated (GPT-4o) & AI-Generated & Our Image, Our Context & AR & 120 \\
    & & Pinterest & Web & Our Context & AR & \\
    & Complex Visual Perception & BLINK & Dataset & Val & En & 1,422 \\
    & Real-world Spatial Understanding & RealWorldQA & Dataset & Test & En & 624 \\
    & Multi-image understanding & MMT-MI-Bench & Dataset & Val & En & 764 \\
    & & MuirBench & Dataset & Test & En & 300 \\
    & Object-level Perception & COCO & Dataset & Test & AR & 60 \\
    & & ImageNet & Dataset & Test & AR &  \\
    & & Mocheg & Dataset & Test & AR &  \\
    & & Snli-Ve & Dataset & Test & AR &  \\
    \hline
    OCR and Document Understanding (7,931)& Scanned Documents & ArabicDatasetOCR & Dataset & - & AR & 480 \\
    & TextVQA & MTVQA & Dataset & Test & AR & 703 \\
    & Scene & EvArEST & Dataset & - & AR & 1,217 \\
    & Books & HAHTR* Dataset & Dataset & - & AR & 40 \\
    & PPTs (OCR) & ISI-PPT-Dataset & Dataset & - & AR & 2,354 \\
    & PPTs (VQA) & & Dataset & - & AR & 711 \\
    & KHATT & &Dataset & & AR & 1,400 \\
    & Scanned Newsletters (VQA) & PATD & Dataset & - & AR & 506 \\
    & OCR Lines & PATS-01 & Dataset & - & AR & 520 \\
    \hline
    Chart and Diagram  & ChartVQA & Dataset & - & En & 745 \\
    \&Understanding (2,820) &Diagrams Understanding & MMMU (Diagrams) & Dataset, Python Charts & Val & En & 255 \\
    & & ICON-QA & Dataset & Val & AR & 1,481 \\
    & AI-Generated (Claude 3.5) & AI-Generated & Our Image, Our Context & AR & 258 \\
    & Pinterest & Web & Our Context & AR & - \\
    & BCE-Arabic & Dataset & Our Context & AR & - \\
    & Tables & BCE-Arabic & Dataset & Our Context & AR & 81 \\
    & &Excel & Created & Our Context & AR & - \\
    \hline
    Video Understanding & Countries/Landmarks & Pexel & Web & Our Context & AR & 111 \\
    & Occasions & Pexel & Web & Our Context & AR & - \\
    & Video-MME & Video-MME & Dataset & Val & En & 654 \\
    \hline
    Cultural-Specific Understanding (1,285 QA) & Celebrities & Arab-Celeb-Dataset & Dataset & Our Context & AR & 444 \\
    & Food & Arabic-Food-101, Pexel & Dataset & Our Context & AR & 347 \\
    & Countries/Landmarks & Pexel & & Our Context & AR & 494 \\
    \hline
    Medical Imaging (506 QA) & Basic Medical Science & MMMU & Dataset & Val + Dev & En & 154 \\
    & Clinical Medicine & MMMU & Dataset & Val + Dev & En & - \\
    & Public Health & MMMU & Dataset & Val + Dev & En & - \\
    & Pharmacy & MMMU & Dataset & Val + Dev & En & - \\
    & Diagnosis & MMMU & Dataset & Val + Dev & En & - \\
    & Medical Understanding & MMT-MI-Bench & Dataset & Val & En & 78 \\
    & Basic Medical Science & MMMU Pro & Dataset & Test & En & 274 \\
    \hline
    AgroVQA & Agriculture VQA & AgroGPT & Dataset & Our Context & AR & 769 \\
    \hline
    Remote Sensing Understanding & GeoData VQA & GeoVQA & Dataset & Val & En & 709 \\
    \hline
    & & & & & & Total QA: 30,419 \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Overview of the CAMEL-Bench dataset, including existing datasets, web-generated content, language, and the number of QA pairs.}}
    \label{tab:camel_bench}
\end{table*}

